Revisiting Membership Problems in Subclasses of Rational Relations

We revisit the membership problem for subclasses of rational relations over finite and infinite words: Given a relation R in a class C_2, does R belong to a smaller class C_1? The subclasses of rational relations that we consider are formed by the deterministic rational relations, synchronous (also called automatic or regular) relations, and recognizable relations. For almost all versions of the membership problem, determining the precise complexity or even decidability has remained an open problem for almost two decades. In this paper, we provide improved complexity and new decidability results. (i) Testing whether a synchronous relation over infinite words is recognizable is NL-complete (PSPACE-complete) if the relation is given by a deterministic (nondeterministic) omega-automaton. This fully settles the complexity of this recognizability problem, matching the complexity of the same problem over finite words. (ii) Testing whether a deterministic rational binary relation is recognizable is decidable in polynomial time, which improves a previously known double exponential time upper bound. For relations of higher arity, we present a randomized exponential time algorithm. (iii) We provide the first algorithm to decide whether a deterministic rational relation is synchronous. For binary relations the algorithm even runs in polynomial time.

==> app-pq.tex <==
	%!TEX root = main.tex
\lempq*

\begin{proof}
The algorithm proceeds as follows.
As a first step we compute for each $q \in Q$ the coarsest refinement $S_q$ of all partitions that are induced by \emph{simple} cycles on $q$.
Check for every $1 \le i < j \le k$ if there exists a simple cycle $q \xrightarrow{\bm{v}} q$ such that $|v_i| \ne |v_j|$
and if so, store it as a constraint that $i$ and $j$ are in different blocks.
Then $S_q$ is the coarsest partition of $[1,k]$ that fulfills all stored constraints.
Note that the existence of a simple cycle $q \xrightarrow{\bm{v}} q$ with $|v_i| \ne |v_j|$ can be checked in nondeterministic logspace
by storing the current length difference of the words in the $i$-th and $j$-th component on the guessed path in a counter whose value is bounded by $|Q|$.

We claim that $P_q = S_{q_1} \sqcap \dots \sqcap S_{q_n}$ 
where $q_1,\dots,q_n$ are the states from which $q$ is reachable.
By definition, $P_q$ is finer than $S_{q_1} \sqcap \dots \sqcap S_{q_n}$.
For the other direction let $P$ be a partition induced by a cycle $c$ from which $q$ is reachable.
For the sake of contradiction assume that there exist $1 \le i < j \le k$ that are in different blocks in $P$ but in the same block in $S_{q_\ell}$ for all $\ell \in [1,n]$.
Since any cycle contains a simple cycle, there exists a simple cycle $p \xrightarrow{\bm{v}} p$ that is contained in $c$.
By assumption, it holds that $|v_i| = |v_j|$ which means that after removing $p \xrightarrow{\bm{v}} p$ from $c$, 
the cycle $c$ still induces a partition where $i$ and $j$ are in different blocks.
Furthermore, $q$ is still reachable from $c$.
We can repeat this argument until $c$ is a simple cycle inducing a partition where $i$ and $j$ are in different blocks, a contradiction.
\end{proof}
